Inverse-Weighted Survival Games

Deep models trained through maximum likelihood have achieved state-of-the-art results for survival analysis. Despite this training scheme, practitioners evaluate models under other criteria, such as binary classification losses at a chosen set of time horizons, e.g. Brier score (BS) and Bernoulli log likelihood (BLL). Models trained with maximum likelihood may have poor BS or BLL since maximum likelihood does not directly optimize these criteria. Directly optimizing criteria like BS requires inverse-weighting by the censoring distribution. However, estimating the censoring model under these metrics requires inverse-weighting by the failure distribution. The objective for each model requires the other, but neither are known. To resolve this dilemma, we introduce Inverse-Weighted Survival Games. In these games, objectives for each model are built from re-weighted estimates featuring the other model, where the latter is held fixed during training. When the loss is proper, we show that the games always have the true failure and censoring distributions as a stationary point. This means models in the game do not leave the correct distributions once reached. We construct one case where this stationary point is unique. We show that these games optimize BS on simulations and then apply these principles on real world cancer and critically-ill patient data.

==> Inverse-Weighted Games (neurips camera-ready)/preamble/abbrevs.tex <==
\newtheorem{thmdef}{Definition}
\newtheorem{thmlem}{Lemma}
\newtheorem{thmcol}{Corollary}
\newtheorem{thmprop}{Proposition}
\newtheorem{thmthm}{Theorem}
\newtheorem{thmappthm}{Theorem}
\newtheorem{thmasmp}{Assumption}
\newtheorem{thmcorr}{Corollary}

\newtheorem{thmappdef}{Definition}
\renewcommand{\thethmappdef}{A\arabic{thmappdef}}
\newtheorem{thmappasmp}{Assumption}
\renewcommand{\thethmappasmp}{A\arabic{thmappasmp}}
\newtheorem{thmapplem}{Lemma}
\renewcommand{\thethmapplem}{A\arabic{thmapplem}}
\newtheorem{thmappcol}{Corollary}
\renewcommand{\thethmappcol}{A\arabic{thmappcol}}



\newenvironment{thmproof}[1][Proof]{\begin{trivlist}
\item[\hskip \labelsep {\textit{#1.}}]}{\end{trivlist}}
\newenvironment{thmproofsketch}[1][Proof sketch]{\begin{trivlist}
\item[\hskip \labelsep {\textit{#1.}}]}{\end{trivlist}}
% \newtheorem{proposition}{Proposition}

\def\bff{\boldsymbol{f}}
% \def\implies{\longrightarrow}
\def\bu{\mathbf{u}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bE{\mathbf{E}}
\def\bw{\mathbf{w}}
\def\cP{\mathcal{P}}
\def\bv{\mathbf{v}}
\def\hbu{\hat{\bu}}
\def\hbv{\hat{\bv}}
\def\balpha{\boldsymbol{\alpha}}
\def\bbeta{\boldsymbol{\beta}}
\def\bmu{\boldsymbol{\mu}}
\def\bgamma{\boldsymbol{\gamma}}
\def\bdelta{\boldsymbol{\delta}}
% \def\E{\mathbb{E}}
\def\E{\mathop{\mathbb{E}}} % redef to make it an operator
% \def\U{\mathcal{U}}
\def\cd{\mathcal{D}}
\def\cg{\mathcal{G}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cL{\mathcal L}
\def\cD{\mathcal D}
\def\cC{\mathcal C}
\def\cI{\mathcal I}
\def\cT{\mathcal T}
\def\cX{\mathcal X}
\def\cY{\mathcal Y}
\def\cH{\mathcal H}
\def\cU{\mathcal U}
\def\cS{\mathcal S}
\def\cF{\mathrm{G}}
\def\cFL{\mathrm{F}_{Lip(1)}}
\def\cx{\mathcal x}
\def\cR{\mathcal{R}}
\def \R{\mathbb{R}}
\def \pFr {p^{F}_\Phi(r,t)}
\def \pCr {p^{CF}_\Phi(r,t)}
\def \epehe{\epsilon_{\text{PEHE}}}
\def \eate{\epsilon_{\text{ATE}}}
\def \eatt{\epsilon_{\text{ATT}}}
\def \eclass{\epsilon_{\text{Class}}}
\def \epehenn{{\epehe}_{nn}}

\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\pc}{p^{t=0}}
\newcommand{\pt}{p^{t=1}}
\newcommand{\dPhi}{\frac{\partial \Phi(x)}{\partial x}}
\newcommand{\dPsi}{\frac{\partial \Psi(r)}{\partial r}}

\newcommand{\errTC}{\mathbb{E}_T \left[\text{err}_{\Phi,h}(C)\right]}
\newcommand{\errTT}{\mathbb{E}_T \left[\text{err}_{\Phi,h}(T)\right]}
\newcommand{\errCC}{\mathbb{E}_C \left[\text{err}_{\Phi,h}(C)\right]}
\newcommand{\errCT}{\mathbb{E}_C \left[\text{err}_{\Phi,h}(T)\right]}

% \newcommand{\errTC}{\mathbb{E}_T \left[\text{err}_C(\Phi,h)\right]}
% \newcommand{\errTT}{\mathbb{E}_T \left[\text{err}_T(\Phi,h)\right]}
% \newcommand{\errCC}{\mathbb{E}_C \left[\text{err}_C(\Phi,h)\right]}
% \newcommand{\errCT}{\mathbb{E}_C \left[\text{err}_T(\Phi,h)\right]}

\newcommand{\lyth}{\ell_{h,\Phi}(x,t)}
\newcommand{\lyxzeroh}{\ell_{h,\Phi}(x,0)}
\newcommand{\lyxoneh}{\ell_{h,\Phi}(x,1)}
\newcommand{\lyzeroh}{\ell_{h,\Phi}(r,0)}
\newcommand{\lyoneh}{\ell_{h,\Phi}(r,1)}

\newcommand{\Jphix}{\frac{\partial \Phi (x)}{\partial x}}
\newcommand{\GP}{\Gamma_\Phi}
\def\diag{\mbox{diag}}


\def\transu{\Delta\bu}
\def\transv{\Delta\bv}
\def\pr{\mbox{Pr}}



==> Inverse-Weighted Games (neurips camera-ready)/preamble/preamble.tex <==
% \RequirePackage[l2tabu, orthodox]{nag}
% \documentclass{article}

% % FONTS
% \usepackage[T1]{fontenc}

% % Replace default Latin Modern typewriter with its proportional counterpart
% % http://www.tug.dk/FontCatalogue/lmoderntypewriterprop/
% \renewcommand*\ttdefault{lmvtt}


% %%% OPTION 1 - Fourier Math + New Century Schoolbook + ParaType Sans

% % % Import Fourier Math (this imposes its own New Century Schoolbook type)
% % % http://www.ctan.org/tex-archive/fonts/fouriernc/
% % \usepackage{fouriernc}
% % \usepackage{amsmath}
% % % Replace with TeX Gyre Schola version of New Century Schoolbook (must scale!)
% % % http://www.tug.dk/FontCatalogue/tgschola/
% % \usepackage[scale=0.92]{tgschola}
% % \usepackage[scaled=0.88]{PTSans}

% %% OPTION 2 - MathDesign Math + Bitstream Charter + ParaType Sans

% % Import MathDesign (this brings along Bitstream Charter)
% % http://www.ctan.org/tex-archive/fonts/mathdesign/
%\usepackage[bitstream-charter]{mathdesign}


%\usepackage{charter}
% \usepackage{amssymb} % only one of this or the above line should be uncommented


%\usepackage{amsmath}
% \usepackage[scaled=0.92]{PTSans}

% \newtheorem{thmcorr}{Corollary}

% % %%% OPTION 3 - MTPRO 2 Math + Termes Times + ParaType Sans

% \usepackage{tgtermes}
% \usepackage{amsmath}
% \usepackage[subscriptcorrection,
%             amssymbols,
%             mtpbb,
%             mtpcal,
%             nofontinfo  % suppresses all warnings
%            ]{mtpro2}
% \usepackage{scalefnt,letltxmacro}
% \LetLtxMacro{\oldtextsc}{\textsc}
% \renewcommand{\textsc}[1]{\oldtextsc{\scalefont{1.10}#1}}
% \usepackage[scaled=0.92]{PTSans}

% % GEOMETRY
% \usepackage[
%   paper  = letterpaper,
%   left   = 1.65in,
%   right  = 1.65in,
%   top    = 1.0in,
%   bottom = 1.0in,
%   ]{geometry}

% COLOR
\usepackage[usenames,dvipsnames]{xcolor}
% \definecolor{shadecolor}{gray}{0.9}

% SPACING and TEXT
%\usepackage[final,expansion=alltext]{microtype} % remove for xetex
% \usepackage[english]{babel}
% \usepackage[parfill]{parskip}
% \usepackage{afterpage}
% \usepackage{framed}

%redefine the leftbar environment to accept a width and coloring options
% \renewenvironment{leftbar}[1][\hsize]
% {%
%   \def\FrameCommand
%   {%
%     {\color{Gray}\vrule width 3pt}%
%     \hspace{10pt}%
%     %\hspace{0pt}\fboxsep=\FrameSep\colorbox{black!10}%
%   }%
%   \MakeFramed{\hsize#1\advance\hsize-\width\FrameRestore}%
% }%
% {\endMakeFramed}
% 
% % define a paragraph header function
% \DeclareRobustCommand{\parhead}[1]{\textbf{#1}~}
% 
% % EDITING
% % line numbering in left margin
% \usepackage{lineno}
% % \renewcommand\linenumberfont{\normalfont
%                             %  \footnotesize
%                             %  \sffamily
%                             %  \color{SkyBlue}}
% % ragged paragraphs in right margin
% \usepackage{ragged2e}
% \DeclareRobustCommand{\sidenote}[1]{\marginpar{
%                                     \RaggedRight
%                                     \textcolor{Plum}{\textsf{#1}}}}
% % paragraph counter in right margin
% \newcommand{\parnum}{\bfseries\P\arabic{parcount}}
% \newcounter{parcount}
% \newcommand\p{%
%     \stepcounter{parcount}%
%     \leavevmode\marginpar[\hfill\parnum]{\parnum}%
% }
% % paragraph helper
% \DeclareRobustCommand{\PP}{\textcolor{Plum}{\P} }
% 
% % COUNTERS
% \renewcommand{\labelenumi}{\color{black!67}{\arabic{enumi}.}}
% \renewcommand{\labelenumii}{{\color{black!67}(\alph{enumii})}}
% \renewcommand{\labelitemi}{{\color{black!67}\textbullet}}

% FIGURES
\usepackage{graphicx}
\usepackage[labelfont=bf]{caption}
% \usepackage[format=hang]{subcaption}

% TABLES
\usepackage{booktabs}

% ALGORITHMS
% \usepackage[algoruled]{algorithm2e}
\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\normalsize}

% BIBLIOGRAPHY
% \usepackage[numbers]{natbib}

% ACRONYMS
\usepackage[acronym,shortcuts,smallcaps,nowarn,nohypertypes={acronym,notation}]{glossaries}



% \makeglossaries

% COLOR DEFINITIONS
\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}

% LISTINGS DEFINTIONS
\lstdefinestyle{mystyle}{
    commentstyle=\color{OliveGreen},
    keywordstyle=\color{BurntOrange},
    numberstyle=\tiny\color{black!60},
    stringstyle=\color{MidnightBlue},
    basicstyle=\ttfamily,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=mystyle}


% HYPERREF
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=MidnightBlue}
\hypersetup{linkcolor=MidnightBlue}
\hypersetup{urlcolor=MidnightBlue}

% CLEVEREF must come after HYPERREF
\usepackage[nameinlink]{cleveref}


\usepackage{tikz}
\usetikzlibrary{shapes,decorations,arrows,calc,arrows.meta,fit,positioning}
\tikzset{
    -Latex,auto,node distance =1 cm and 1 cm,semithick,
    state/.style ={circle, draw, minimum width = 0.7 cm},
    detstate/.style ={rectangle, draw, minimum width = 0.7 cm, minimum height = 0.7 cm},
    % hidden/.style ={circle, draw, inner sep=0.04cm,fill,node contents={},},
    point/.style = {circle, draw, inner sep=0.04cm,fill,node contents={}},
    bidirected/.style={Latex-Latex,dashed},
    el/.style = {inner sep=2pt, align=left, sloped}
}

\usepackage{wrapfig}
\usepackage{mathtools}
\def\nyu{New York University}
\def\cs{Computer Science}
\def\cims{Courant Institute}
\def\cds{Center for Data Science}
\def\ny{NY, NY}


==> Inverse-Weighted Games (neurips camera-ready)/preamble/preamble_acronyms.tex <==
\newacronym{KL}{kl}{Kullback-Leibler}
\newacronym{ELBO}{elbo}{\emph{evidence lower bound}}
\newacronym{POPELBO}{pop-elbo}{\emph{population evidence lower bound}}

\newacronym{SVI}{svi}{stochastic variational inference}
\newacronym{conc}{conc}{concordance}


\newacronym{svm}{svm}{svm}

\newacronym{BUMPVI}{bump-vi}{bumping variational inference}

\newacronym{GMM}{gmm}{Gaussian mixture model}
\newacronym{LDA}{lda}{latent Dirichlet allocation}

\newacronym{SUTVA}{sutva}{stable unit treatment value assumption}

\newacronym{KSD}{ksd}{{kernelized Stein discrepancy}}
\newacronym{KCC-SD}{kcc-sd}{kernelized complete conditional Stein discrepancy}


\newacronym{OPVI}{opvi}{operator variational inference}
\newacronym{SVGD}{svgd}{Stein variational gradient descent}

\newacronym{vde}{vde}{variational decoupling}
\newacronym{cfn}{cfn}{control-function method}
\newacronym{gcfn}{gcfn}{generalized control-function method}
\newacronym{2sls}{2sls}{two-stage least-squares method}
\newacronym{gmm}{gmm}{generalized method of moments}
\newacronym{iv}{iv}{instrumental variable}
\newacronym{cdf}{cdf}{cumulative distribution function}
\def\cdir{conditioning direction}
\def\edir{exogenizing direction}
\def\zm{ignorability methods}
\def\zv{confounding-variation}
\newcommand{\epsv}{{\gls{iv}-variation}}
\newcommand{\epsm}{{\gls{iv} methods}}


%  calibration
%\newacronym{ours}{X-calibration}{eXplicit calibration}
\newacronym{x-cal}{x-cal}{explicit calibration}
\newcommand{\xcaled}{\textsc{x-calibrated}}
% \newacronym{ours-ed}{x-calibrated}{eXplicit calibration}
\newacronym{d-cal}{d-calibration}{distributional calibration}
\newacronym{d-cal-short}{d-cal}{d-cal}



\newacronym{nll}{nll}{negative log likelihood}
\newacronym{ipcw}{ipcw}{inverse probability of censor-weighting}
\newacronym{bs}{bs}{Brier score}

\newacronym{fbs}{fbs}{F Brier score}
\newacronym{gbs}{gbs}{G Brier score}

\newacronym{fbscw}{fbscw}{Weighted F Brier score}
\newacronym{gbscw}{gbscw}{Weighted G Brier score}


\newacronym{bl}{bl}{Bernoulli likelihood}
\newacronym{bll}{bll}{Bernoulli log likelihood}
\newacronym{auc}{auc}{area under curve}
\newacronym{km}{km}{Kaplan-Meier}

\newacronym{gan}{gan}{Generative Adversarial Network}



\newacronym{support}{support}{Study to Understand Prognoses Preferences Outcomes and Risks of Treatment}
\newacronym{metabric}{metabric}{Molecular Taxonomy of Breast Cancer International Consortium}
\newacronym{rott}{rott}{Rotterdam Tumor Bank}
\newacronym{gbsg}{gbsg}{German Breast Cancer Study Group}
\newacronym{rott-gbsg}{rott. \& gbsg}{Rotterdam \& GBSG}
\newacronym{flchain}{flchain}{The Assay Of Serum Free Light Chain}
\newacronym{nwtco}{nwtco}{National Wilm’s Tumor Study}
\newacronym{crash2}{crash-2}{Clinical Randomization of an Antifibrinolyticin Significant Hemorrhage 2}
\newacronym{uw-dcal}{uw-dcal}{uniform-weighted d-cal}
\newacronym{ipcw-dcal}{ipcw-dcal}{\gls{ipcw} d-cal}
\newacronym{ipcw-xcal}{ipcw-xcal}{\gls{ipcw} x-cal}
\newacronym{ibs}{ibs}{integrated brier score}
\newacronym{ipcw-ibs}{ipcw-ibs}{\gls{ipcw}-\gls{ibs}}

\newacronym{crps}{crps}{continuous ranked probability score}
\newacronym{s-crps}{s-crps}{Survival-\acrshort{crps}}
\newacronym{ifd}{ifd}{individual failure distribution}

\newacronym{hl}{hl}{Hosmer-Lemeshow}
\newacronym{gb}{gb}{Grønnesby-Borgan}
\newacronym{dn}{dn}{D’Agostino-Nam}

\newacronym{ni}{ni}{Not-Interpolated}
\newacronym{i}{i}{Interpolated}
\newacronym{mimic-iii}{mimic-iii}{Medical Information Mart for Intensive Care}
\newacronym{mnist}{mnist}{Modified National Institute of Standards and Technology database}
\newacronym{tcga}{tcga}{The Cancer Genome Atlas}
\newacronym{mtlr}{mtlr}{Multi-Task Logistic Regression}
\newacronym{aft}{aft}{Accelerated Failure Times}

==> Inverse-Weighted Games (neurips camera-ready)/preamble/preamble_math.tex <==

\DeclareRobustCommand{\mb}[1]{\ensuremath{\boldsymbol{\mathbf{#1}}}}

% \define@key{mafx@}{mathbold}[\mathbold]{\let#1=\mafx@mathbold}

\DeclareRobustCommand{\KL}[2]{\ensuremath{\textrm{KL}\left(#1\;\|\;#2\right)}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareRobustCommand{\dho}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}

\renewcommand{\mid}{~\vert~}

\newcommand{\mba}{\mb{a}}
\newcommand{\mbb}{\mb{b}}
\newcommand{\mbc}{\mb{c}}
\newcommand{\mbd}{\mb{d}}
\newcommand{\mbe}{\mb{e}}
\newcommand{\mbg}{\mb{g}}
\newcommand{\mbh}{\mb{h}}
\newcommand{\mbi}{\mb{i}}
\newcommand{\mbj}{\mb{j}}
\newcommand{\mbk}{\mb{k}}
\newcommand{\mbl}{\mb{l}}
\newcommand{\mbm}{\mb{m}}
\newcommand{\mbn}{\mb{n}}
\newcommand{\mbo}{\mb{o}}
\newcommand{\mbp}{\mb{p}}
\newcommand{\mbq}{\mb{q}}
\newcommand{\mbr}{\mb{r}}
\newcommand{\mbs}{\mb{s}}
\newcommand{\mbt}{\mb{t}}
\newcommand{\mbu}{\mb{u}}
\newcommand{\mbv}{\mb{v}}
\newcommand{\mbw}{\mb{w}}
\newcommand{\mbx}{\mb{x}}
\newcommand{\mby}{\mb{y}}
\newcommand{\mbz}{\mb{z}}

\newcommand{\vx}{x}
\newcommand{\vd}{d}
\newcommand{\vtau}{\mathtt{\tau}}
\newcommand{\vt}{t}
\newcommand{\vs}{{s}}
\newcommand{\vk}{{k}}

\newcommand{\mbA}{\mb{A}}
\newcommand{\mbB}{\mb{B}}
\newcommand{\mbC}{\mb{C}}
\newcommand{\mbD}{\mb{D}}
\newcommand{\mbE}{\mb{E}}
\newcommand{\mbF}{\mb{F}}
\newcommand{\mbG}{\mb{G}}
\newcommand{\mbH}{\mb{H}}
\newcommand{\mbI}{\mb{I}}
\newcommand{\mbJ}{\mb{J}}
\newcommand{\mbK}{\mb{K}}
\newcommand{\mbL}{\mb{L}}
\newcommand{\mbM}{\mb{M}}
\newcommand{\mbN}{\mb{N}}
\newcommand{\mbO}{\mb{O}}
\newcommand{\mbP}{\mb{P}}
\newcommand{\mbQ}{\mb{Q}}
\newcommand{\mbR}{\mb{R}}
\newcommand{\mbS}{\mb{S}}
\newcommand{\mbT}{\mb{T}}
\newcommand{\mbU}{\mb{U}}
\newcommand{\mbV}{\mb{V}}
\newcommand{\mbW}{\mb{W}}
\newcommand{\mbX}{\mb{X}}
\newcommand{\mbY}{\mb{Y}}
\newcommand{\mbZ}{\mb{Z}}

\newcommand{\mbalpha}{\mb{\alpha}}
\newcommand{\mbbeta}{\mb{\beta}}
\newcommand{\mbdelta}{\mb{\delta}}
\newcommand{\mbepsilon}{\mb{\epsilon}}
\newcommand{\mbchi}{\mb{\chi}}
\newcommand{\mbeta}{\mb{\eta}}
\newcommand{\mbgamma}{\mb{\gamma}}
\newcommand{\mbiota}{\mb{\iota}}
\newcommand{\mbkappa}{\mb{\kappa}}
\newcommand{\mblambda}{\mb{\lambda}}
\newcommand{\mbmu}{\mb{\mu}}
\newcommand{\mbnu}{\mb{\nu}}
\newcommand{\mbomega}{\mb{\omega}}
\newcommand{\mbphi}{\mb{\phi}}
\newcommand{\mbpi}{\mb{\pi}}
\newcommand{\mbpsi}{\mb{\psi}}
\newcommand{\mbrho}{\mb{\rho}}
\newcommand{\mbsigma}{\mb{\sigma}}
\newcommand{\mbtau}{\mb{\tau}}
\newcommand{\mbtheta}{\mb{\theta}}
\newcommand{\mbupsilon}{\mb{\upsilon}}
\newcommand{\mbvarepsilon}{\mb{\varepsilon}}
\newcommand{\mbvarphi}{\mb{\varphi}}
\newcommand{\mbvartheta}{\mb{\vartheta}}
\newcommand{\mbvarrho}{\mb{\varrho}}
\newcommand{\mbxi}{\mb{\xi}}
\newcommand{\mbzeta}{\mb{\zeta}}



\newcommand{\mbDelta}{\mb{\Delta}}
\newcommand{\mbGamma}{\mb{\Gamma}}
\newcommand{\mbLambda}{\mb{\Lambda}}
\newcommand{\mbOmega}{\mb{\Omega}}
\newcommand{\mbPhi}{\mb{\Phi}}
\newcommand{\mbPi}{\mb{\Pi}}
\newcommand{\mbPsi}{\mb{\Psi}}
\newcommand{\mbSigma}{\mb{\Sigma}}
\newcommand{\mbTheta}{\mb{\Theta}}
\newcommand{\mbUpsilon}{\mb{\Upsilon}}
\newcommand{\mbXi}{\mb{\Xi}}

\newcommand{\dif}{\mathop{}\!\mathrm{d}}
% \newcommand{\diag}{\textrm{diag}}
\newcommand{\supp}{\textrm{supp}}

%\newcommand{\E}{\mathbb{E}}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\Var}{\mathbb{V}\textrm{ar}}
\newcommand{\bbH}{\mathbb{H}}

\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}

% \newcommand{\cO}{\mathcal{O}}
% \newcommand{\cL}{\mathcal{L}}
% \newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cQ}{\mathcal{Q}}
% \newcommand{\cS}{\mathcal{S}}

% \newcommand{\cN}{\mathcal{N}}
% \newcommand{\cT}{\mathcal{T}}

% \newcommand{\E}{\mathbb{E}}
\newcommand{\Cov}{\mathbb{C}\textrm{ov}}

\newcommand{\cB}{\mathcal{B}}
\newcommand{\Gam}{\textrm{Gam}}
\newcommand{\InvGam}{\textrm{InvGam}}


\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\A}{\mathcal{A}}
% \newcommand{\cU}{\mathcal{U}}
\newcommand{\Func}{\mathcal{F}}
\newcommand{\Ker}{\mathcal{K}}
\newcommand{\St}{\mathcal{S}}
\newcommand{\Kernel}{\mathcal{K}_{k}}
\newcommand{\euclid}{\mathbb{R}}
\newcommand{\score}{s^{p}}
\newcommand{\hz}{\hat{\mbz}}
\newcommand{\hy}{\hat{\mby}}
\newcommand{\he}{\hat{\mbepsilon}}
\newcommand{\hg}{\hat{g}}
\newcommand{\DO}{\text{do}}
% \def\do{\text{do}}
% \renewcommand{\ht}{\hat{t}}


\newcommand{\g}{\mid}
\newcommand{\gtight}{\vert}

\newtheorem{prop}{Proposition}
% \newtheorem{thmdef}{Definition}
% \newtheorem{lemma}{Lemma}
\newtheorem{corr}{Corollary}
\newtheorem{thm}{Theorem}
\newtheorem{appthm}{Theorem}
\newtheorem{asmp}{Assumption}

\crefname{lemma}{lemma}{lemmas}
\crefname{prop}{proposition}{propositions}
\newcommand\myeq{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily c}}}{=}}}


% \newcommand{\indicator}{\mathbbm{1}}
\DeclareRobustCommand{\indicator}[1]{\ensuremath{\mathbbm{1}\left[#1\right]}}


%\DeclareRobustCommand{\largertilde}[1]{\ensuremath{\overset{\sim}{\mathcal{#1}}}}

\DeclareRobustCommand{\largertilde}[1]{\ensuremath{\stackrel{\sim}{\smash{\mathcal{#1}}\rule{0pt}{1.1ex}}}}

\newcommand{\dcal}{\cL}
\newcommand{\uwdcal}{\cL_{UW}}


\newcommand{\softdcal}{\hat{\cL}_{UW,\gamma}}
\newcommand{\softupperdcal}{\hat{\cL}_{UW,\gamma}^+}
\newcommand{\softupperdcaluncensored}{\hat{\cL}_{\gamma}^+}

\newcommand{\ipcwdcal}{\cL_{CW}}
\newcommand{\softipcwdcal}{\hat{\cL}_{CW,\gamma}}


\newcommand{\softupperipcwdcal}{\hat{\cL}_{CW,\gamma}^+}



\newcommand{\ipcwdcalfailure}{\cL_{CW}^{\text{fail}}}
\newcommand{\ipcwdcalcensor}{\cL_{CW}^{\text{cens}}}



\newcommand{\softupperipcwdcalfailure}{\hat{\cL}_{CW,\gamma}^{+\text{fail}}}
\newcommand{\softupperipcwdcalcensor}{\hat{\cL}_{CW,\gamma}^{+\text{cens}}}

\newcommand{\tonetrue}{\theta^\star_{T1}}
\newcommand{\ttwotrue}{\theta^\star_{T2}}
\newcommand{\tthreetrue}{\theta^\star_{T3}}
\newcommand{\tonehat}{\hat{\theta}_{T1}}
\newcommand{\ttwohat}{\hat{\theta}_{T2}}
\newcommand{\tthreehat}{\hat{\theta}_{T3}}
\newcommand{\tktrue}{\theta^\star_{tk}}
\newcommand{\tkhat}{\hat{\theta}_{tk}}
\newcommand{\tKtrue}{\theta^\star_{tK}}
\newcommand{\tKhat}{\hat{\theta}_{tK}}
\newcommand{\titrue}{\theta^\star_{Ti}}
\newcommand{\tihat}{\hat{\theta}_{Ti}}
\newcommand{\tkplusonetrue}{\theta^\star_{T(k+1)}}
\newcommand{\tkplusonehat}{\hat{\theta}_{T(k+1)}}
\newcommand{\conetrue}{\theta^\star_{C1}}
\newcommand{\ctwotrue}{\theta^\star_{C2}}
\newcommand{\cthreetrue}{\theta^\star_{C3}}
\newcommand{\cktrue}{\theta^\star_{Ck}}
\newcommand{\ckhat}{\hat{\theta}_{Ck}}
\newcommand{\cKtrue}{\theta^\star_{CK}}
\newcommand{\cKhat}{\hat{\theta}_{CK}}
\newcommand{\citrue}{\theta^\star_{Ci}}
\newcommand{\cihat}{\hat{\theta}_{Ci}}
\newcommand{\ckplusonetrue}{\theta^\star_{C(k+1)}}
\newcommand{\ckplusonehat}{\hat{\theta}_{C(k+1)}}
\newcommand{\conehat}{\hat{\theta}_{C1}}
\newcommand{\ctwohat}{\hat{\theta}_{C2}}
\newcommand{\cthreehat}{\hat{\theta}_{C3}}
